CHORD: Category-level Hand-held Object Reconstruction via Shape Deformation

In daily life, humans utilize hands to manipulate objects. Modeling the shape of objects that are manipulated by the hand is essential for AI to comprehend daily tasks and to learn manipulation skills. However, previous approaches have encountered difficulties in reconstructing the precise shapes of hand-held objects, primarily owing to a deficiency in prior shape knowledge and inadequate data for training. As illustrated, given a particular type of tool, such as a mug, despite its infinite variations in shape and appearance, humans have a limited number of 'effective' modes and poses for its manipulation. This can be attributed to the fact that humans have mastered the shape prior of the 'mug' category, and can quickly establish the corresponding relations between different mug instances and the prior, such as where the rim and handle are located. In light of this, we propose a new method, CHORD, for Category-level Hand-held Object Reconstruction via shape Deformation. CHORD deforms a categorical shape prior for reconstructing the intra-class objects. To ensure accurate reconstruction, we empower CHORD with three types of awareness: appearance, shape, and interacting pose. In addition, we have constructed a new dataset, COMIC, of category-level hand-object interaction. COMIC contains a rich array of object instances, materials, hand interactions, and viewing directions. Extensive evaluation shows that CHORD outperforms state-of-the-art approaches in both quantitative and qualitative measures. Code, model, and datasets are available at https://kailinli.github.io/CHORD.

==> tables/normaldepth_prior.tex <==
\begin{table}[h]
    \begin{center}
    \rowcolors{3}{WhiteGray}{White}
\begin{minipage}[!htp]{0.42\linewidth}
        \begin{center}
            \resizebox{1.0\linewidth}{!}{
            \makeatletter\def\@captype{table}\makeatother
            \setlength{\tabcolsep}{10pt}{
                \begin{tabular}{cc|c}
                \toprule
                \nstargt & \dstargt & CD $\downarrow$\\
                \midrule
                 \redcross & \redcross & 7.88   \\
                 \greencheck & \redcross & 8.03  \\
                 \redcross & \greencheck & 7.58 \\
                 \greencheck & \greencheck & 7.45 \\
                \midrule
                 \bluecheck & \bluecheck & \textbf{7.07} \\
                \bottomrule
                \end{tabular}
            }
            }\vspace{-3pt}
        \caption{\expref{E} Comparison of \model with different appearance features. }
            \label{table:normal_depth_ablation}
        \end{center}
        \end{minipage}
        \quad
\begin{minipage}[!htp]{0.48\linewidth}
    \begin{center}
       \includegraphics[width=0.9\linewidth]{figures/prior.pdf}
        \label{fig:prior_axis}
    \captionof{figure}{Illustration of the \objprior (obtained from DIT) of the six categories in \dataset dataset. }
    \end{center}
\end{minipage}
    \end{center}\vspace{-2.5em}
\end{table}



==> tables/prior_pose.tex <==
\begin{table}[t]
    \begin{center}
        \begin{minipage}[!htp]{0.45\linewidth}
        \begin{center}
            \resizebox{1.0\linewidth}{!}{
            \makeatletter\def\@captype{table}\makeatother
            \setlength{\tabcolsep}{10pt}{
            \rowcolors{2}{WhiteGray}{White}
                \begin{tabular}{l|c}
                \toprule
                Methods & CD $\downarrow$\\
                \midrule
                 Voxel Mean & 10.27   \\
                 DeepSDF Mean & 9.41  \\
                 DIT \cite{Zheng2020DeepImpTemp} & \textbf{7.99} \\
                \bottomrule
                \end{tabular}
            }
        }
        \caption{\expref{C} Comparison of the different methods for generating \objprior.}
        \label{table:prior_ablation}
        \end{center}
        \end{minipage}
        \;
        \begin{minipage}[!htp]{0.50\linewidth}
        \begin{center}
            \resizebox{1.0\linewidth}{!}
            {
            \makeatletter\def\@captype{table}\makeatother
            \setlength{\tabcolsep}{1mm}{
                \setlength{\aboverulesep}{0pt}
                \setlength{\belowrulesep}{0pt}
                \rowcolors{2}{WhiteGray}{White}
                \setlength{\tabcolsep}{10pt}{
                    \begin{tabular}{l|c}
                    \toprule
                    Methods & CD $\downarrow$ \\
                    \midrule
                     \queryx to  \joints \& \handverts dist. &  10.00  \\
                     \queryx's signed dist. &  7.50 \\
                     \ensuremath{\transfinv_b(\queryx)} w/o global &  7.41  \\
                     \ensuremath{\transfinv_b(\queryx)} w/ global &  \textbf{7.27}  \\
                    \bottomrule
                    \end{tabular}
                }}
            }
            \caption{\expref{D} Comparison of different methods for embedding hand pose into \threednet.} 
            \label{table:pose_ablation}
        \end{center}

    \end{minipage}
    \end{center}\vspace{-2.5em}
\end{table}
